Provably Efficient Exploration in Quantum Reinforcement Learning with Logarithmic Worst-Case Regret

While quantum reinforcement learning (RL) has attracted a surge of attention recently, its theoretical understanding is limited. In particular, it remains elusive how to design provably efficient quantum RL algorithms that can address the exploration-exploitation trade-off. To this end, we propose a novel UCRL-style algorithm that takes advantage of quantum computing for tabular Markov decision processes (MDPs) with $S$ states, $A$ actions, and horizon $H$, and establish an $\mathcal{O}(\mathrm{poly}(S, A, H, \log T))$ worst-case regret for it, where $T$ is the number of episodes. Furthermore, we extend our results to quantum RL with linear function approximation, which is capable of handling problems with large state spaces. Specifically, we develop a quantum algorithm based on value target regression (VTR) for linear mixture MDPs with $d$-dimensional linear representation and prove that it enjoys $\mathcal{O}(\mathrm{poly}(d, H, \log T))$ regret. Our algorithms are variants of UCRL/UCRL-VTR algorithms in classical RL, which also leverage a novel combination of lazy updating mechanisms and quantum estimation subroutines. This is the key to breaking the $\Omega(\sqrt{T})$-regret barrier in classical RL. To the best of our knowledge, this is the first work studying the online exploration in quantum RL with provable logarithmic worst-case regret.

==> note.tex <==
\section{Interaction Procedure}

Given an MDP $\mathcal{M} = (\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, H)$, define the Hilbert space $\caH_S, \caH_A, \caH_R$ to embed the superpositions of state/action/rewards. Assume the basis for $\caH_S, \caH_A, \caH_R$ are $\{\ket{s}\}_{s \in \caS}, \{\ket{a}\}_{a \in \caA}, \{\ket{0}, \ket{1}\}$. We hope to learn the optimal policy of $\caM$ with the help of quantum tools.

For a policy $\pi(\cdot \mid s)$, we assume the ability to construct a unitary $\Pi(\pi)$ such that 

\begin{align}
    \Pi(\pi) : \ket{s}\ket{0}_{\caA} \to \sum_{a} \sqrt{\pi(a \mid s)} \ket{s}\ket{a}.
\end{align}

The agent interacts with $\caM$ through two oracles $\caP, \caR$% (we may have to add some auxiliary input to $\bm{M}$, but we omit it for simplicity):

\begin{align}
\caP & : \ket{s} \ket{a} \ket{0} \to \ket{s} \ket{a} \otimes \left(\sum_{s' \in \caS} \sqrt{P(s' \mid s, a)} \ket{s'}\right) \\
\caR & : \ket{s} \ket{a} \ket{0} \to \ket{s} \ket{a} \otimes \ket{R(s,a)}
\end{align}

%where $r(s, a) = \dbP(\caR(s, a) = 1)$.

The agent is able to interact with $\caM$ for $K$ episodes. At the beginning of each episode, the agent is able to construct the initial state $\ket{s_1}$. However, \textbf{he is not able to prepare any $\ket{s}$ for $s \in \caS$}. All he can do after obtain $\ket{s_1}$ is to query $\caP, \caR$ for at most $H$ steps, and perform quantum operations through this process.



\section{Concentration}

\subsection{Quantum mean estimation in \citet{cornelissen2022near}}
Given a $d$ dimensional random variable $X$ with $\EE[X] = \mu \in \RR^d$ and $\text{Cov}(X) = \Sigma$, we can construct estimator $\tilde{\mu}$, using $n$ samples, such that
\$
\|\tilde{\mu}-\mu\|_{2} \leqslant\left\{\begin{array}{ll}\sqrt{\frac{\operatorname{Tr}(\Sigma)}{n}} & \text { if } n \le d, \\ \frac{\sqrt{d \operatorname{Tr(\Sigma )}} \log d}{n} & \text { if } n>d.\end{array}\right.
\$

%In quantum language: For each $(s, a)$, $X$ now is a $S$-dimensional vector, such that $X$ takes value $\bm{1}_{s'}$ with probability $P(s' \mid s, a)$. Therefore, we only need a quantum oracle $O_{s, a}$ such that 

%$$ O_{s, a}: \ket{0} \to \sum_{s'} \sqrt{P(s' \mid s, a)}\ket{s'}$$

\subsection{Quantum amplitude estimation}

Following \citet{van2021quantum}, given an oracle $U$ that quantize the randomness of distribution $p$: 

$$ U\ket{0} = \sum_{i=1}^d \sqrt{p_i}\ket{i}. $$

We can obtain an estimate $\hat{p}$ such that $\|\hat{p} - p\|_1 \leq d \log (d / \delta)/n$ holds with probability $1 - \delta$ using $O(n)$ queries to $U$ and $U^{-1}$.

%\subsection{Improved amplitude }

\subsection{Application to RL}
%Fix $(s, a)$, given $n(s, a)$ samples, we construct an estimator $\tilde{P}(\cdot \mid s, a) \in \RR^S$ 
%\$
%&\| \tilde{P}(\cdot \mid s, a) - P(\cdot \mid s, a) \|_2 
% \le  \left\{\begin{array}{ll} \sqrt{\frac{S}{n(s,a)}} & \text { if } n(s, a) \le d, \\ \frac{S}{n(s,a)} & \text { if } n(s, a) >d.\end{array}\right.
%\$
%&\| \tilde{P}(\cdot \mid s, a) - P(\cdot \mid s, a) \|_1 
% \le \frac{S}{n(s,a)}.
%\$



%\section{Algorithm}

\begin{algorithm}[h]
	\caption{Quantum UCRL2}
		\begin{algorithmic}[1]
		    \STATE \textbf{Initialize:} $i_{s, a} = \tilde{n}(s, a) = 0$ for all $(s, a)$
      \FOR{$k = 1, \cdots, K$}
      \FOR{$h = H, \cdots, 1$}
      \STATE $Q_h^k(\cdot, \cdot) = r(\cdot, \cdot) + \tilde{\PP}V_{h+1}^k(\cdot, \cdot) + b_h(\cdot, \cdot)$
      \STATE $V_h^k(s) = \max_{a \in \cA} Q_h^k(s, a)$
      \STATE $\pi_h^k(x) = \argmax_{a} Q_h^k(s, a)$
      \ENDFOR
      \STATE Prepare $\Pi(\pi^k)$
      \FOR{$h = 1, \cdots, H$}
      \STATE Prepare $\ket{s_1}$, and query $\caP$ for $h$ times to obtain quantum state $\phi^k_h = \sum_{s} \sqrt{d^{\pi^k}_h(s)} \ket{s}$
      \STATE Measure $\phi^k_h$ and receive the state $s_h^k$, query $\caP$ on $\Pi_h(\pi^k) \ket{s_h^k}$ and store the result in $\mathcal{D}(s_h^k, \pi^k_h(s_h^k))$.
      \IF{$\tilde{n}(s_h^k, a_h^k) = 2^{i_{s_h^k, a_h^k}}$}
      \STATE Update $\tilde{P}(\cdot \mid s_h^k, a_h^k)$ using $\tilde{n}(s_h^k, a_h^k)$ sample (with $\tilde{n}(s_h^k, a_h^k)$ access to the $O_{s_h^k, a_h^k}$ oracle and do measurement)
      \STATE $i_{s_h^k, a_h^k} = i_{s_h^k, a_h^k} + 1$
      \STATE $\tilde{n}(s_h^k, a_h^k) = 0$
      \ENDIF
      \ENDFOR
      \ENDFOR
      \end{algorithmic}
\end{algorithm}

\section{Analysis}

\subsection{Optimism}

Fix $(s, a)$, given $n^k(s, a)$ samples, we construct an estimator $\tilde{P}(\cdot \mid s, a) \in \RR^S$ 
\$
 | \tilde{\PP}V(s, a) - \PP V(s, a) | &\le \| \tilde{P}(\cdot \mid s, a) - P(\cdot \mid s, a) \|_1 \cdot \|V\|_{\infty} \\
 & \le H \cdot \| \tilde{P}(\cdot \mid s, a) - P(\cdot \mid s, a) \|_1 \\
 & \leq \frac{HS \log (S^2A \log T / \delta)}{n^k(s, a)} \\
% & \lesssim  \left\{\begin{array}{ll} \frac{HS}{\sqrt{\tilde{n}(s,a)}}, & \text { if } \tilde{n}(s, a) \le S, \\ \frac{H\sqrt{S^3}}{\tilde{n}(s,a)} & \text { if } \tilde{n}(s, a) >S.\end{array}\right. \\
%& \lesssim  \left\{\begin{array}{ll} \frac{HS}{\sqrt{n(s,a)}}, & \text { if } n(s, a) \le S, \\ \frac{H\sqrt{S^3}}{n(s,a)} & \text { if } n(s, a) >S.\end{array}\right. \\
& := b^k(s, a).
\$

\begin{remark}
    Let $n(s, a)$ be the total number of visiting $(s, a)$. Assume $\tilde{P}(\cdot \mid s, a)$ is calculated by $\tilde{n}(s, a)$ samples, then $n(s, a) \in [\tilde{n}(s, a), 2\tilde{n}(s, a)]$. Therefore, we can replace $\tilde{n}(s, a)$ by $n(s, a)$ in the last inequality. 
\end{remark}

\subsection{Regret Analysis}

It holds that the high probability regret can be decomposed as 
\$
\mathrm{Regret}(T) &\le H \EE \Big[ \sum_{k = 1}^K \sum_{h = 1}^H 2b(s_h^k, a_h^k)\Big] \\
%& \le HS \cdot S^2 A + H S^{1.5} \cdot SA \log T \\
%&= HS^3A + HS^{2.5} A \log T.
& \leq  2H (HS \log (S^2A \log T / \delta) \times SA \log (SAHT/\delta) + SAH \log (SAHT / \delta))  \\
&= \tilde{O}(H^2 S^2 A \log (T / \delta)).
\$

\section{Lower Bound}

Previous paper studying the lower bound of approximating $\pi^*$ shows that the query complexity is $\Omega(S\sqrt{A} H^{1.5} / \epsilon)$ even with a generative model. Here we do not have a generative model, so the lower bound query complexity of approximating $\pi^*$ will be at least $\Omega(S\sqrt{A} H^{1.5} / \epsilon)$ in our setting. 

The $\sqrt{A}$ lower bound essentially comes from the fact that the query complexity of finding argmax in $A$ items are $\Theta(\sqrt{A})$ (e.g. in multi-armed bandits), and their lower bound are proved by reducing to $O(S)$ bandits problem. However, we need to tackle the hardness of exploration in our setting, this is likely to incur at least $O(SA)$ query complexity.

Important facts: the construction cannot reduce to multiarmed bandits; the main hardness comes from the diffculty of doing exploration in \textbf{states}.

\subsection{A possible construction}

Consider $S$ states divided into two layers, each consisting of $S/2$ states. 

For the $i$-th state in the second layer, it is a terminal state (i.e. transit to himself), the rewards of exactly one action is $1/i$, the others are 0.

For each state in the first layer, it connects to $A$ different states in the second layer.

%where the last inequality uses the facts that $n(s, a) \le S$ will occur at most $S$ times for any $(s, a)$ and the pigeon-hole principle.

\section{Linear Function Approximation}

We study the linear mixture MDP, which is defined as follows.
\begin{definition}[Linear Mixture MDP]
    We say an MDP $(\cS, \cA, H, \cP, R)$ is a linear mixture MDP if there exists a known feature map $\psi: \cS \times \cA \times \cS \rightarrow \RR^d$ and unknown vectors $\{\theta_h \in \RR^d\}_{h \in [H]}$ such that 
    \$
    \cP_h(s' \given s, a) = \psi(s, a, s')^\top \theta_h
    \$
    for all $(s, a, s', h) \in \cS \times \cA \times \cS \times [H]$.
\end{definition}

\begin{algorithm}[h]
	\caption{Quantum VTR}
		\begin{algorithmic}[1]
      \FOR{phase $k = 1, \cdots$}
      \STATE Calculate $\{\hat{\theta}_h^k\}_{h \in [H]}$
      \STATE Obtain $\pi^k = \{\pi_h^k\}_{h \in [H]}$ via the optimistic planning oracle
      \STATE Prepare $\Pi(\pi^k)$
      \STATE Calculate $\{\hat{\phi}_h^k\}_{h \in [H]}$ by Algorithm \ref{}, which are estimators of $\phi_h^{k} = \EE_{\pi^k} \int_{s' \in \cS} \psi(s_h, \pi_h^k(s_h), s') V_{h+1}^k(s')$
      \STATE Set $\epsilon_k = \max_{h \in [H]} \|\hat{\phi}_h^k\|_{(\Lambda_h^k)^{-1}}$ 
      \STATE Execute $\pi^k$ for $\tilde{\cO}(1/\epsilon_k)$ times and calculate $\{y_h^k\}_{h \in [H]}$ (by quantum mean estimation), which is an estimator of $\{\PP_h V_{h+1}^k\}_{h \in [H]}$
      \ENDFOR
      \end{algorithmic}
\end{algorithm}

\begin{definition}[Optimistic Planning] 
  Given parameters $(\{\hat{\theta_h}\}_{h \in [H]}, \{\Lambda_h\}_{h \in [H]}, \beta)$, the optimistic planning oracle solves the following problem:
  \begin{equation}
  \begin{aligned} \label{eq:planning}
      & \max  V_1(s_1)  \\
      \text{s.t. } &Q_h(\cdot, \cdot) = r_h(\cdot, \cdot) + \phi_{V_{h+1}}(\cdot, \cdot)^\top \theta_h , \quad \forall h \in [H] \\
      & V_h(\cdot) = \max_{a \in \cA} Q_h(\cdot, a) , \quad \forall h \in [H], \quad V_{H+1}(\cdot) = 0, \\
      & \| \theta_h - \hat{\theta}_h \|_{\Lambda_h} \le \beta, \quad \forall h \in [H] .
  \end{aligned}
  \end{equation}
\end{definition}



\newpage 

\paragraph{Question:}
How many samples do we need to calculate $\hat{\phi}_h^k$ such that
\$
\|\hat{\phi}_h^k - \phi_h^k\|_2 \le \| \hat{\phi}_h^k \|_{{(\Lambda_h^k)}^{-1}} .
\$

\paragraph{Potential solution:}
First of all, note that for any $x, y \in \dbR^d$, it holds that 

\begin{align}
\left|\|x\|_{{(\Lambda_h^k)}^{-1}} - \|y\|_{{(\Lambda_h^k)}^{-1}}\right| \leq \left\|{{(\Lambda_h^k)}^{-1/2}}(x - y)\right\|_2 \leq \|x - y\|_2.
\end{align}

We construct a series of estimator $\{\hat{\phi}_{h,n}^k\}_{n=1}^\infty$ such that 

$$ \left\|\hat{\phi}_{h,n}^k - \phi_h^k\right\|_2 \leq 2^{-n}$$

until the condition

\begin{align}
\left\|\hat{\phi}_{h,n}^k\right\|_{{(\Lambda_h^k)}^{-1}} - 2^{-n} - 2^{-(n+1)} \geq 2^{-(n+1)}
\end{align}

is satisfied. 

This condition ensures that 

\begin{align}
\left\|\hat{\phi}_{h,n+1}^k - \phi_h^k\right\|_2 & \leq 2^{-(n+1)} \\
& \leq \left\|\hat{\phi}_{h,n}^k\right\|_{{(\Lambda_h^k)}^{-1}} - 2^{-n} - 2^{-(n+1)} \\
& \leq \left\|\phi_{h}^k\right\|_{{(\Lambda_h^k)}^{-1}} - 2^{-(n+1)} \\
& \leq \left\|\hat{\phi}_{h,n+1}^k\right\|_{{(\Lambda_h^k)}^{-1}}.
\end{align}

Thus $\hat{\phi}_{h,n+1}^k$ will be a valid estimator.

On the other hand, we know that as long as $n > n_0$ such that 

\begin{align}
\left\|\hat{\phi}_{h,n_0}^k\right\|_{{(\Lambda_h^k)}^{-1}} - 2^{-n_0} - 2^{-(n_0+1)} & \geq \left\|\phi_{h}^k\right\|_{{(\Lambda_h^k)}^{-1}} - 2^{-(n_0 - 1)} - 2^{-(n_0 + 1)} \\
& \geq 2^{-(n_0 + 1)} \\
 2^{n_0} & \geq \frac{3}{\left\|\phi_{h}^k\right\|_{{(\Lambda_h^k)}^{-1}}}.
\end{align}

The condition will be triggered when $n = n_0$. The total number of quantum queries will be $O(\left\|\phi_{h}^k\right\|_{{(\Lambda_h^k)}^{-1}}^{-1})$.
\iffalse
The term in the regret is 

$$ \dbE_{\pi}[b_h^k(s_h, a_h)] = \dbE_{\pi}\left[\|\phi_h^k(s_h, a_h)\|_{(\Lambda_h^k)^{-1}}\right], $$

which is greater than 

$$ \|\dbE_{\pi}[\phi_h^k(s_h, a_h)]\|_{(\Lambda_h^k)^{-1}} $$

as the case in linear bandits.
\fi


\paragraph{Regret Analysis}

Following \citet{cai2020provably}, we have 
\$
\EE[\mathrm{Regret}(T)] &\le  \EE \Big[ \sum_{k = 1}^K V_1^k(s_1) - V_1^{\pi^k}(s_1) \Big] \\
& = \sum_{h = 1}^H \sum_{k = 1}^K \EE_{\pi^k} [ \hat{\PP}_h^k V_{h+1}^k(s_h, a_h) - \PP_h V_{h+1}^k(s_h, a_h) ] \\
& = \sum_{h = 1}^H \sum_{k = 1}^K (\phi_h^k)^\top (\hat{\theta}_h^k - \theta_h) \\
& \approx \sum_{h = 1}^H \sum_{k = 1}^K (\hat{\phi}_h^k)^\top (\hat{\theta}_h^k - \theta_h) ,
\$
where $\phi_h^k = \EE_{\pi^k} \phi(s_h, a_h)$. Moreover, by Cauchy-Schwarz inequality, we obtain
\$
\sum_{h = 1}^H \sum_{k = 1}^K (\hat{\phi}_h^k)^\top (\hat{\theta}_h^k - \theta_h) \le \sum_{h = 1}^H \sum_{k = 1}^K \|\hat{\phi}_h^k\|_{(\Lambda_h^k)^{-1}} \cdot  \| \hat{\theta}_h^k - \theta_h \|_{\Lambda_h^k} .  
\$

\paragraph{Regret Caused by Estimating $\phi_h^k$}

We need $\cO(H/\max_{h} \|\phi_h^k\|_{\Lambda_h^k})$ to estimate $\{\phi_h^k\}$, the regret is upper bounded by
\$
\cO(H/\max_{h} \|\phi_h^k\|_{\Lambda_h^k}) \cdot \beta_k \sum_{h = 1}^H \|\phi_h^k\|_{(\Lambda_h^k)^{-1}} \le \cO(H^2 \beta_k).
\$


\paragraph{Regression}

\$
\hat{\theta}_h^k = \argmin_{\theta} \sum_{\tau = 1}^{k - 1} \frac{1}{\epsilon_\tau^2} \| (\hat{\phi}_h^\tau)^\top \theta - y_h^\tau \|_2^2 + \lambda I_d,
\$
where $y_h^\tau$ is the quantum estimator of $\EE_{\pi^\tau} [\PP_h V_{h+1}^\tau(s_h, a_h)]$. Hence, we have
\$
\hat{\theta}_h^k - \theta_h = (\Lambda_h^k)^{-1} \Big( \sum_{\tau = 1}^{k - 1} \frac{1}{\epsilon_\tau^2} \cdot \phi_h^\tau \cdot \big( y_h^\tau - (\hat{\phi}_h^\tau)^{\top} \theta_h  \big) \Big) - \lambda (\Lambda_h^k)^{-1} \theta_h,
\$
which further implies that 
\$
\| \hat{\theta}_h^k - \theta_h \|_{\Lambda_h^k} \le  \Big\| \sum_{\tau = 1}^{k - 1} \frac{1}{\epsilon_\tau^2} \cdot \phi_h^\tau \cdot \big( y_h^\tau - (\hat{\phi}_h^\tau)^{\top} \theta_h  \big) \Big\|_{(\Lambda_h^k)^{-1}} + \sqrt{\lambda d} .
\$
If we have 
\$
y_h^\tau - (\hat{\phi}_h^\tau)^{\top} \theta_h  & = \underbrace{y_h^\tau - ({\phi}_h^\tau)^{\top} \theta_h}_{\text{quantum estimator}} + \underbrace{({\phi}_h^\tau)^{\top} \theta_h - (\hat{\phi}_h^\tau)^{\top} \theta_h}_{\text{approximation error}} \approx \|\hat{\phi}_h^\tau\|_{(\Lambda_h^k)^{-1}} = \epsilon_\tau,
\$
we can follow \citet{wan2022quantum} to obtain that 
\$
\| \hat{\theta}_h^k - \theta_h \|_{\Lambda_h^k} \le \sqrt{\lambda d} + \sqrt{d k} := \beta_k.
\$

So the regret induced by phase $k$ is roughly 
\$
\tilde{\cO}(1/\epsilon_k) \cdot \beta_k \sum_{h = 1}^H \|\hat{\phi}_h^k\|_{(\Lambda_h^k)^{-1}} \le H \beta_k,
\$
where we use the fact that $\epsilon_k = \max_{h \in [H]} \|\hat{\phi}_h^k\|_{(\Lambda_h^k)^{-1}}$.
